Deep learning generalizes because the parameter-function map is biased towards simple functions

Deep neural networks (DNNs) generalize remarkably well without explicit regularization even in the strongly over-parametrized regime where classical learning theory would instead predict that they would severely overfit. While many proposals for some kind of implicit regularization have been made to rationalise this success, there is no consensus for the fundamental reason why DNNs do not strongly overfit. In this paper, we provide a new explanation. By applying a very general probability-complexity bound recently derived from algorithmic information theory (AIT), we argue that the parameter-function map of many DNNs should be exponentially biased towards simple functions. We then provide clear evidence for this strong simplicity bias in a model DNN for Boolean functions, as well as in much larger fully connected and convolutional networks applied to CIFAR10 and MNIST. As the target functions in many real problems are expected to be highly structured, this intrinsic simplicity bias helps explain why deep networks generalize well on real world problems. This picture also facilitates a novel PAC-Bayes approach where the prior is taken over the DNN input-output function space, rather than the more conventional prior over parameter space. If we assume that the training algorithm samples parameters close to uniformly within the zero-error region then the PAC-Bayes theorem can be used to guarantee good expected generalization for target functions producing high-likelihood training sets. By exploiting recently discovered connections between DNNs and Gaussian processes to estimate the marginal likelihood, we produce relatively tight generalization PAC-Bayes error bounds which correlate well with the true error on realistic datasets such as MNIST and CIFAR10 and for architectures including convolutional and fully connected networks.

==> Deep learning generalizes because the parameter-function map is biased towards simple functions (ICLR)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Deep learning generalizes because the parameter-function map is biased towards simple functions (ICLR)/suppinfo.tex <==
\section{Basic Experimental details}
\label{methods}

In the main experiments of the paper we used two classes of architectures. Here we describe them in more detail.

\begin{itemize}
    \item Fully connected networks (FCs), with varying number of layers. The size of the hidden layers was the same as the input dimension, and the nonlinearity was ReLU. The last layer was a single Softmax neuron. We used default Keras settings for initialization (Glorot uniform).
    \item Convolutional neural networks (CNNs), with varying number of layers. The number of filters was $200$, and the nonlinearity was ReLU. The last layer was a fully connected single Softmax neuron. The filter sizes alternated between $(2,2)$ and $(5,5)$, and the padding between SAME and VALID, the strides were $1$ (same default settings as in the code for \cite{garriga2018convnets}). We used default Keras settings for initialization (Glorot uniform).
    % \item Residual neural networks (ResNets), with varying number of layers. We used 'v2' residual blocks, with the same default settings as in the code for [[]]). We used default Keras settings for initialization (Glorot uniform)
\end{itemize}

In all experiments in Section~\ref{experiments} we trained with SGD with a learning rate of $0.01$, and early stopping when the accuracy on the whole training set reaches $100\%$.

In the experiments where we learn Boolean functions with the smaller neural network with $7$ Boolean inputs and one Boolean output (results in Figure~\ref{fig:generror_LZ}), we use a variation of SGD similar to the method of adversarial training proposed by Ian Goodfellow~\cite{goodfellow2014explaining}. We chose this second method because SGD often did not find a solution with $0$ training error for all the Boolean functions, even with many thousand iterations. By contrast, the adversarial method succeeded in almost all cases, at least for the relatively small neural networks which we focus on here. 

We call this method \emph{adversarial SGD}, or \emph{advSGD}, for short. In SGD, the network is trained using the average loss of a random sample of the training set, called a \emph{mini-batch}. In advSGD, after every training step, the classification error for each of the training examples in the mini-batch is computed, and a moving average of each of these classification errors is updated. This moving average gives a score for each training example, measuring how ``bad'' the network has recently been at predicting this example. Before getting the next mini-batch, the scores of all the examples are passed through a softmax to determine the probability that each example is put in the mini-batch. This way, we force the network to focus on the examples it does worst on. For advSGD, we also used a batch size of $10$.

In all experiments we used binary cross entropy as the loss function. We found that Adam could learn Boolean functions with the smaller neural network as well, but only when choosing the mean-squared error loss function.

For the algorithms to approximate the marginal likelihood in Section~\ref{gaussian_processes}, we used a Bernoulli likelihood with a probit link function to approximate the true likelihood (given by the Heaviside function)

\section{Testing the approximations to the Gaussian process marginal likelihood}
\label{testing_approx_ml}

In Figure~\ref{fig:GP_NN_approx}, we show results comparing the empirical frequency of labellings for a sample of $10$ random MNIST images, when these frequencies are obtained by sampling parameters of a neural network (with a Gaussian distribution with parameters $\sigma_w=\sigma_b=1.0$), versus that calculated using two methods to approximate the marginal likelihood of the Gaussian process corresponding to the neural network architecture we use. We compare the Laplacian and expectation-propagation approximations.(see \cite{rasmussen2004gaussian} for a description of the algorithms)  The network has 2 fully connected hidden layers of $784$ ReLU neurons each. 

\begin{figure}[tph]
\centering
% \begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=0.57\textwidth]{GP_NN_1e7_m10_EPLapvfreq.png}
% \caption{\label{fig:GP_NN_approx_10}for a sample of $m=10$ inputs, $\sigma_w,\sigma_b=1.0$}
% \end{subfigure}
% \begin{subfigure}[b]{0.49\textwidth}
% \includegraphics[width=\textwidth]{GP_NN_1e7_m20_EPLapvfreq.png}
% \caption{\label{fig:GP_NN_approx_20}for a sample of $m=20$ inputs,  $\sigma_w,\sigma_b=100.0$}
% \end{subfigure}

\caption{\label{fig:GP_NN_approx}Comparing the empirical frequency of different labellings for a sample of $10$ MNIST images obtained from randomly sampling parameters from a neural neural network, versus the approximate marginal likelihood from the corresponding Gaussian process. Orange dots correspond to the expectation-propagation approximation, and blue dots to the Laplace approximation. The network has 2 fully connected hidden layers of $784$ ReLU neurons each. The weight and bias variances are $1.0$.}
\end{figure}

\section{The choice of variance hyperparameters}
\label{choice_variance}

One limitation of our approach is that it depends on the choice of the variances of the weights and biases used to define the equivalent Gaussian process. Most of the trends shown in the previous section were robust to this choice, but not all. For instance, the bound for MNIST was higher than that for fashion-MNIST for the fully connected network, if the variance was chosen to be $1.0$.

In Figures~\ref{fig:varsweeps_cnn} and \ref{fig:varsweeps_fc}, we show the effect of the variance hyperparameters on the bound. Note that for the fully connected network, the variance of the weights $\sigma_w$ seems to have a much bigger role. This is consistent with what is found in \cite{lee2017deep}. Furthermore, in \cite{lee2017deep} they find, for smaller depths, that the neural network Gaussian process behaves best above $\sigma_w\approx 1.0$, which marks the transition between two phases characterized by the asymptotic behavior of the correlation of activations with depth. This also agrees with the behaviour of the PAC-Bayes bound. For CIFAR10, we find that the bound is best near the phase transition, which is also compatible with results in \cite{lee2017deep}. For convolutional networks, we found sharper transitions with weight variance, and an larger dependence on bias variance (see Fig.~\ref{fig:varsweeps_cnn}). For our experiments, we chose variances values above the phase transition, and which were fixed for each architecture.

The best choice of variance would correspond to the Gaussian distribution best approximates the behaviour of SGD. We measured the variance of the weights after training with SGD and early stopping (stop when $100\%$ accuracy is reached) from a set of initializations, and obtained values an order of magnitude smaller than those used in the experiments above. Using these variances gave significantly worse bounds, above $50\%$ for all levels of corruption.

This measured variance does not necessarily measure the variance of the Gaussian prior that best models SGD, as it also depends on the shape of the zero-error surface (the likelihood function on parameter space). However, it might suggest that SGD is biased towards better solutions in paramater space, giving a stronger/better bias than that predicted only by the parameter-function map with Gaussian sampling of parameters. One way this could happen is if SGD is more likely to find flat (global) ``minima''\footnote{Note that the notion of minimum is not well defined given that the region of zero error seems to be mostly flat and connected (\cite{sagun2017empirical,draxler2018essentially})} than what is expected from near-uniform sampling of the region of zero-error (probability proportional to volume of minimum). This may be one of the main sources of error in our approach. A better understanding of the relation between SGD and Bayesian parameter sampling is needed to progress on this front (\cite{lee2017deep,matthews2018gaussian}).

% \subsection{Dependence of PAC-Bayes bound on variance hyperparameters}
% \label{bound_variance}

\begin{figure}[tph]
\centering
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{mnist-fashion_bound_vs_sigmaw_sigmab1_fc.png}
\caption{\label{fig:sigmaw_fashion_fc}fashion-MNIST}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{mnist-fashion_bound_vs_sigmab_sigmaw1_fc.png}
\caption{\label{fig:sigmab_fashion_fc}fashion-MNIST}
\end{subfigure}

\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{mnist_bound_vs_sigmaw_sigmab1_fc.png}
\caption{\label{fig:sigmaw_mnist_fc}MNIST}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{mnist_bound_vs_sigmab_sigmaw1_fc.png}
\caption{\label{fig:sigmab_mnist_fc}MNIST}
\end{subfigure}

\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{cifar_bound_vs_sigmaw_sigmab1_fc.png}
\caption{\label{fig:sigmaw_cifar_fc}CIFAR10}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{cifar_bound_vs_sigmab_sigmaw1_fc.png}
\caption{\label{fig:sigmab_cifar_fc}CIFAR10}
\end{subfigure}
\caption{\label{fig:varsweeps_fc} \emph{Dependence of PAC-Bayes bound on variance hyperparameters}. We plot the value of the PAC-Bayes bound versus the standard deviation parameter for the weights and biases, for a sample of $10000$ instances from different datasets, and a two-layer fully connected network (with the layers of the same size as input). The fixed parameter is put to $1.0$ in all cases.}
\end{figure}

\begin{figure}[tph]
\centering
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{mnist-fashion_bound_vs_sigmaw_sigmab1_cnn.png}
\caption{\label{fig:sigmaw_fashion_cnn}fashion-MNIST}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{mnist-fashion_bound_vs_sigmab_sigmaw1_cnn.png}
\caption{\label{fig:sigmab_fashion_cnn}fashion-MNIST}
\end{subfigure}

\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{mnist_bound_vs_sigmaw_sigmab1_cnn.png}
\caption{\label{fig:sigmaw_mnist_cnn}MNIST}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{mnist_bound_vs_sigmab_sigmaw1_cnn.png}
\caption{\label{fig:sigmab_mnist_cnn}MNIST}
\end{subfigure}

\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{cifar_bound_vs_sigmaw_sigmab1_cnn.png}
\caption{\label{fig:sigmaw_cifar_cnn}CIFAR10}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{cifar_bound_vs_sigmab_sigmaw1_cnn.png}
\caption{\label{fig:sigmab_cifar_cnn}CIFAR10}
\end{subfigure}
\caption{\label{fig:varsweeps_cnn} \emph{Dependence of PAC-Bayes bound on variance hyperparameters}. PAC-Bayes bound versus the standard deviation parameter for the weights and biases, for a sample of $10000$ instances from different datasets, and a four-layer convolutional network. The fixed parameter is put to $1.0$ in all cases.}
\end{figure}

\section{Details on the experiments comparing the probability of finding a function by SGD and neural network Gaussian processes}
\label{sgd_vs_bayes_details}

Here we describe in more detail the experiments carried out in Section~\ref{sgd_vs_bayes} in the main text. We aim to compare the probability $P(f|S)$ of finding a particular function $f$ when training with SGD, and when training with approximate Bayesian inference (ABI), given a training set $S$. We consider this probability, averaged over of training sets, to look at the properties of the algorithm rather than some particular training set. In particular, consider a sample of $N$ training sets $\{S_1,...,S_N\}$ of size $118$. Then we are interested in the quantity (which we refer to as \emph{average probability of finding function $f$}):

\begin{align*}
    \langle P(f) \rangle := \frac{1}{N} \sum_{i=1}^n P(f|S_i)
\end{align*}

For the SGD-like algorithms, we approximate $P(f|S_i)$ by the fraction of times we obtain $f$ from a set of $M$ random runs of the algorithm (with random initializations too). For ABI, we calculate it as:

\begin{equation*}
P(f|S_i)=\begin{cases}
\frac{P(f)}{P(S_i)} &\mbox{if $f$ consistent with $S_i$} \\ 
0 &\mbox{otherwise} 
\end{cases},
\end{equation*}

\noindent
where $P(f)$ is the prior probability of $f$ computed using the EP approximation of the Gaussian process corresponding to the architecture we use, and $P(S_i)$ is the marginal likelihood of $S_i$ under this prior probability.

In Fig.~\ref{fig:sgd_abi_smallvar}, we show results for the same experiment as in Figure~\ref{fig:sgd_abi_bigvar} in main text, but with lower variance hyperparameters for the Gaussian process, which results in significantly worse correlation.

\begin{figure}[tph]
\centering
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{{SGD_prob_EPapprox_no_single_sample_vs_advsgd_many_84.0_7_40_2_150000_10000_118_no_replace_1.0_1.0_1.0}.png}
\caption{\label{fig:advsgd_abi_smallvar}advSGD. $\rho=0.72$,$p=\expnumber{1}{-6}$}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{{SGD_prob_EPapprox_vs_adam_many_84.0_7_40_2_150000_10000_118_no_replace_1.0_1.0_1.0}.png}
\caption{\label{fig:adam_abi_smallvar}Adam. $\rho=0.66$,$p=\expnumber{2}{-7}$}
\end{subfigure}
\caption{\label{fig:sgd_abi_smallvar} We plot $\langle P(f) \rangle$ for a variant of SGD, versus $\langle P(f) \rangle$ computed using the ABI method described above (which approximates uniform sampling on parameter space on the zero-error region). The Gaussian process parameters (see Section~\ref{gaussian_processes} in main text) are $\sigma_w=1.0$, and $\sigma_b=1.0$. For advSGD, we have removed functions which only appared once in the whole sample, to avoid finite-size effects. In the captions $\rho$ refers to the 2-tailed Pearson correlation coefficient, and $p$ to its corresponding p value.}
\end{figure}


\section{Simplicity bias and the parameter-function map}
\label{param-fun-map-complexity}

An important argument in Section~\ref{why_real_world} in the main text is that the parameter-function map of neural networks should exhibit the basic simplicity bias phenomenolgy recently described in Dingle et al.\ in~\cite{simpbias}.  In this section we briely describe some key results of reference~\cite{simpbias} relevant to this argument.

A computable\footnote{Here computable simply means that all inputs lead to outputs, in other words there is no halting problem.} input-output map $f: I\rightarrow O$, mapping $N_I$ inputs from the set $I$ to $N_O$ outputs $x$ from the set $O$\footnote{This language of finite input and outputs sets assumes discrete inputs and outputs, either because they are intrinsically discrete, or because they can be made discrete by a coarse-graining procedure.  For the parameter-function maps studied in this paper the set of outputs (the full hypothesis class) is typically naturally discrete, but the inputs are continuous.  However, the input parameters can always be discretised without any loss of generality.} may exhibit simplicity bias if the following restrictions are satisfied (\cite{simpbias}):

1) {\it Map simplicity} The map should have limited complexity, that is its Kolmogorov complexity $K(f)$ should asymptotically satisfy $K(f) + K(n) \ll K(x) + O(1)$, for typical $x \in O$ where $n$ is a measure of the size of the input set (e.g.\ for binary input sequences, $N_I = 2^n$.).  

2) {\it Redundancy}: There should be many more inputs than outputs ($N_I \gg N_O$)  so that the probability $P(x)$ that the map generates output $x$ upon random selection of inputs $\in I$ can in principle vary significantly. 

3) {\it  Finite size} $N_O \gg 1$ to avoid potential finite size effects.

4) {\it Nonlinearity}: The map $f$ must be a nonlinear function since linear functions do not exhibit bias.
% Well, except in trivial cases

5) {\it Well behaved}: The map should not primarily produce pseudorandom outputs (such as the digits of $\pi$), because complexity approximators needed for practical applications will mistakenly label these as highly complex.

%\end{enumerate}

For the deep learning learning systems studied in this paper, the inputs of the map $f$ are the parameters that fix the weights for the particular neural network architecture chosen, and the outputs are the functions that the system produces.  Consider, for example, the configuration for Boolean functions studied in the main text. While the output functions rapidly grow in complexity with increasing size of the input layer, 
%For the parameter-function maps presented in this work, the output sizes are typically of size $>100$ (and much larger for larger networks). On the other hand, 
the map itself can be described with a low-complexity procedure, since it consists of reading the list of parameters, populating a given neural network architecture and evaluating it for all inputs. For reasonable architectures, the information needed to describe the map grows logarithmically with the input dimension $n$, so for large enough $n$, the amount of information required to describe the map will be much less than the information needed to describe a typical function, which requires $2^{2^n}$ bits. % The last step of the map evaluates this network for all possible inputs to output the function in its string representation, and only needs  ${\cal O}(\log(n))$ bits to describe the size of the input.
Thus the Kolmogorov complexity $K(f)$ of this map is asymptotically smaller than the the typical complexity of the output, as required by the map simplicity condition 1) above.

The redundancy condition 2) depends on the network architecture and discretization.  For overparameterised networks, this condition is typically satisfied. In our specific case, where we use floating point numbers for the parameters (input set $I$), and Boolean functions (output set $O$), this condition is clearly satisfied.  Neural nets can represent very large numbers of potential functions (see for example estimates of VC dimension \cite{bartlett2017nearly,baum1989size}), so that condition 3) is also generally satisfied. Neural network parameter-function maps are evidently non-linear, satisfying condition 4). Condition 5) is perhaps the least understood condition within simplicity bias. However, the lack of any function with high probability and high complexity (at least when using LZ complexity), provides some empirical validation. This condition also agrees with the expectation that neural networks will not predict the outputs of a good pseudorandom number generator. One of the implicit assumptions in the simplicity bias framework is that, although true Kolmogorov complexity is always uncomputable, approximations based on well chosen complexity measures perform well for most relevant outputs $x$.  Nevertheless, where and when this assumptions holds is a deep problem for which further research is needed. 

\section{Other complexity measures}
\label{complexity_measures}

One of the key steps to practical application of the simplicity bias framework of Dingle et al.\ in~\cite{simpbias} is the identification of a suitable complexity measure $\tilde{K}(x)$ which mimics aspects of  the (uncomputable) Kolmogorov complexity $K(x)$ for the problem being studied.   
It was shown for the maps in~\cite{simpbias} that several different complexity measures all generated the same qualitative simplicity bias behaviour:
\begin{equation}
P(x) \leq 2^{-(a \tilde{K}(x)+b)}
\end{equation}
but with different values of $a$ and $b$ depending on the complexity measure and of course depending on the map, but independent of output $x$.   Showing that the same qualitative results obtain for different complexity measures is sign of robustness for simplicity bias.

Below we list a number of different descriptional complexity measures which we used, to extend the experiments in Section~\ref{why_real_world} in the main text.

\subsection{Complexty measures}
\label{complexity-measures}

\emph{Lempel-Ziv complexity} (\emph{LZ complexity} for short).
The Boolean functions studied in the main text can be written as binary strings, which makes it possible to use measures of complexity based on finding regularities in binary strings. One of the best is Lempel-Ziv complexity, based on the Lempel-Ziv compression algorithm. It has many nice properties, like asymptotic optimality, and being asymptotically equal to the Kolmogorov complexity for an ergodic source. We use the variation of Lempel-Ziv complexity from~\cite{simpbias} which is based on the 1976 Lempel Ziv algorithm~(\cite{lempel1976complexity}): 
\begin{equation}
K_{LZ}(x) =\begin{cases}
     \log_2(n), &  \hspace*{-0.3cm}  \text{$x=0^n$ or $1^n$}\\
    \log_2(n) [N_w(x_1...x_n) + N_{w}(x_n...x_1)]/2, & \hspace*{-0.2cm} \text{otherwise}
  \end{cases}\label{eq:CLZ}
\end{equation}
where $n$ is the length of the binary string, and $N_w(x_1...x_n)$ is the number of words in the Lempel-Ziv "dictionary" when it compresses output $x$.   The symmetrization makes the measure more fine-grained, and the $\log_2(n)$ factor as well as the value for the simplest strings ensures that they scale as expected for Kolmogorov complexity.  This complexity measure is the primary one used in the main text.

We note that the binary string representation depends on the order in which inputs are listed to construct it, which is not a feature of the function itself. This may affect the LZ complexity,  although for low-complexity input orderings (we use numerical ordering of the binary inputs), it has a negligible effect, so that $K(x)$ will be very close to the Kolmogorov complexity of the function.

\emph{Entropy}. A fundamental, though weak, measure of complexity is the entropy. For a given binary string this is defined as $S=-\frac{n_0}{N}\log_2{\frac{n_0}{N}} -\frac{n_1}{N}\log_2{\frac{n_1}{N}}$, where $n_0$ is the number of zeros in the string, and $n_1$ is the number of ones, and $N=n_0+n_1$. This measure is close to $1$ when the number of ones and zeros is similar, and is close to $0$ when the string is mostly ones, or mostly zeros.
Entropy and $K_{LZ}(x)$ are compared in Fig.~\ref{fig:complexities-correlation}, and in more detail in supplementary note 7 (and supplementary information figure 1) of reference~\cite{simpbias}. They correlate, in the sense that low entropy $S(x)$  means low $K_{LZ}(x)$, but it is also possible to have Large entropy but low  $K_{LZ}(x)$, for example for a string such as $10101010...$. 


\emph{Boolean expression complexity}.  Boolean functions can be compressed by finding simpler ways to represent them.  We used the standard SciPy implementation of the Quine-McCluskey algorithm  to minimize the Boolean function into a small sum of products form, and then defined the number of operations in the resulting Boolean expression as a \emph{Boolean complexity} measure.


\emph{Generalization complexity}. L. Franco et al. have introduced a complexity measure for Boolean functions, designed to capture how difficult the function is to learn and generalize~(\cite{franco2004generalization}), which was used to empirically find that simple functions generalize better in a neural network~(\cite{franco2006generalization}). The measure consists of a sum of terms, each measuring the average over all inputs fraction of neighbours which change the output. The first term considers neighbours at Hamming distance of $1$, the second at Hamming distance of $2$ and so on. The first term is also known (up to a normalization constant) as average sensitivity~(\cite{friedgut1998boolean}). The terms in the series have also been called ``generalized robustness'' in the evolutionary theory literature (\cite{greenbury2016genetic}). Here we use the first two terms, so the measure is:

\begin{align*}
C(f) = C_1(f) + C_2(f),\\
C_1(f) = \frac{1}{2^n n} \sum_{x \in X} \sum_{y \in  \text{Nei}_1(x)} |f(x) - f(y)|, \\
C_1(f) = \frac{2}{2^n n(n-1)} \sum_{x \in X} \sum_{y \in  \text{Nei}_2(x)} |f(x) - f(y)|,
\end{align*}

\noindent
where $\text{Nei}_i(x)$ is all neighbours of $x$ at Hamming distance $i$.

\emph{Critical sample ratio}. A measure of the complexity of a function was introduced in~\cite{arpit2017closer} to explore the dependence of generalization with complexity. In general, it is defined with respect to a sample of inputs as the fraction of those samples which are \emph{critical samples}, defined to be an input such that there is another input within a ball of radius $r$, producing a different output (for discrete outputs). Here, we define it as the fraction of all inputs, that have another input at Hamming distance $1$, producing a different output.

\subsection{Correlation between complexities}
\label{complexities-correlation}

In Fig.~\ref{fig:complexities-correlation}, we compare the different complexity measures against one another.   We also plot the frequency of each complexity; generally more functions are found with higher complexity.
\begin{figure}[htp]
\centering
\includegraphics[width=\textwidth]{complexities_scatter_matrix.png}
\caption{\label{fig:complexities-correlation} Scatter matrix showing the correlation between the different complexity measures used in this paper On the diagonal, a histogram (in grey) of frequency versus complexity is depicted.  The  functions  are from the sample of $10^8$ parameters for the $(7,40,40,1)$ network.}
\end{figure}

\subsection{Probability-complexity plots}
\label{prob-comp-plots}

In Fig.~\ref{fig:simpbias} we show how the probability versus complexity plots look for other complexity measures.  The behaviour is similar to that seen for the LZ complexity measure in Fig~1(b) of  the main text. In Fig.~\ref{fig:prob_comp_dists} %and \ref{fig:prob_comp_layers},
we show probability versus LZ complexity plots for other choices of parameter distributions.
% and network architectures, respectively. 

\begin{figure}[tph]
\centering
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{cnt_100000000_7_40_40_1_relu_freq_BC.png}
\caption{\label{fig:simpbias_Boolcomp}Probability versus Boolean complexity}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{cnt_100000000_7_40_40_1_relu_freq_GC.png}
\caption{\label{fig:simpbias_gencomp}Probability versus generalization complexity}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{cnt_100000000_7_40_40_1_relu_freq_ent.png}
\caption{\label{fig:simpbias_ent}Probability versus entropy}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{cnt_100000000_7_40_40_1_relu_freq_CSR.png}
\caption{\label{fig:simpbias_csr}Probability versus critical sample ratio}
\end{subfigure}
\caption{\label{fig:simpbias}Probability versus different measures of complexity (see main text for Lempel-Ziv), estimated from a sample of $10^8$ parameters, for a network of shape $(7,40,40,1)$. Points with a frequency of $10^{-8}$ are removed for clarity because these suffer from finite-size effects (see \SI~\ref{finite-size-effects}). The measures of complexity are described in \SI~\ref{complexity_measures}. }
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.65\textwidth]{prob_comp_g_sampled_linearscale.png}
\caption{\label{fig:simpbias_LZ_hist} Histogram of functions in the probability versus Lempel-Ziv complexity plane, weighted according to their probability. Probabilities are estimated from a sample of $10^8$ parameters, for a network of shape $(7,40,40,1)$}
\end{figure}

\begin{figure}[tph]
\centering
\begin{subfigure}[t]{0.49\textwidth}
\includegraphics[width=\textwidth]{cnt_1000000_7_20_20_1_relu_gaussian_sample_freq_LZ.png}
\caption{\label{fig:prob_comp_layers_gaussian} }
\end{subfigure}
~
\begin{subfigure}[t]{0.49\textwidth}
\includegraphics[width=\textwidth]{cnt_1000000_7_20_20_1_relu_high_variance_freq_LZ.png}
\caption{\label{fig:prob_comp_layers_high_var} }
\end{subfigure}
\caption{\label{fig:prob_comp_dists} Probability versus LZ complexity for network of shape $(7,40,40,1)$ and varying sampling distributions. Samples are of size $10^7$. (a) Weights are sampled from a Gaussian with variance $1/\sqrt{n}$ where $n$ is the input dimension of each layer. (b) Weights are sampled from a Gaussian with variance $2.5$ }
\end{figure}

\clearpage

\subsection{Effects of target function complexity on learning for different complexity measures}
\label{learning_appendix}

Here we show the effect of the complexity of the target function on learning, as well as other complementary results. Here we compare neural network learning to random guessing, which we call ``unbiased learner''. Note that both probably have the same hypothesis class as we tested that the neural network used here can fit random functions.

The functions in these experiments were chosen by randomly sampling parameters of the neural network used, and so even the highest complexity ones are probably not fully random\footnote{The fact that non-random strings can have maximum LZ complexity is a consequence of LZ complexity being a less powerful complexity measure than Kolmogorov complexity, see e.g.~\cite{estevez2013non}. The fact that neural networks do well for non-random functions, even if they have maximum LZ, suggests that their simplicity bias captures a notion of complexity stronger than LZ.}. In fact, when training the network on truly random functions, we obtain generalization errors equal or above those of the unbiased learner. This is expected from the No Free Lunch theorem, which says that no algorithm can generalize better (for off-training error) uniformly over all functions than any other algorithm (\cite{wolpert1994relationship}).

% Furthermore, the fact that non-random functions

% In Figure~\ref{fig:generror_LZ}, we see that the network performs better than the unbiased algorithm for functions over the whole range of complexities. However, the functions in these experiments were chosen by randomly sampling parameters, and so even the highest complexity ones are probably not random. In fact, when training the network on truly random functions, we obtain generalization errors slightly above those of the unbiased learner, showing that LZ complexity is not powerful enough to fully capture the bias of the network.

\begin{figure}[htp]
\centering
\begin{subfigure}[t]{0.49\textwidth}
 \includegraphics[width=\textwidth]{generalization_errors_LZcomp_40_advSGD_0_5train_larger_font.png}
	\caption{Generalization error of learned functions}
    \label{fig:generror_HC}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
	\includegraphics[width=\textwidth]{LZ_comp_learned_vs_LZ_comp_0_5train.png}
    \caption{Complexity of learned functions}
    \label{fig:HC_HC}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
	\includegraphics[width=\textwidth]{iters_LZ.png}
    \caption{Number of iterations to perfectly fit training set}
    \label{fig:iters_HC}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
	\includegraphics[width=\textwidth]{dists_LZ.png}
    \caption{Net Euclidean distance traveled in parameter space to fit training set}
    \label{fig:dists_HC}
\end{subfigure}
\caption{\label{fig:target_comp_effects}Different learning metrics versus the LZ complexity of the target function, when learning with a network of shape $(7,40,40,1)$. Dots represent the means, while the shaded envelope corresponds to piecewise linear interpolation of the standard deviation, over $500$ random initializations and training sets.}
\end{figure}

\begin{figure}[htp]
\centering
\begin{subfigure}[t]{0.49\textwidth}
 \includegraphics[width=\textwidth]{generalization_errors_GCcomp_40_advSGD_0_5train_larger_font.png}
	\caption{Generalization error of learned functions}
    \label{fig:generror_HC}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
	\includegraphics[width=\textwidth]{GC_comp_learned_vs_GC_comp_0_5train_larger_font.png}
    \caption{Complexity of learned functions}
    \label{fig:HC_HC}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
	\includegraphics[width=\textwidth]{iters_HC.png}
    \caption{Number of iterations to perfectly fit training set}
    \label{fig:iters_HC}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
	\includegraphics[width=\textwidth]{dists_HC.png}
    \caption{Net Euclidean distance traveled in parameter space to fit training set}
    \label{fig:dists_HC}
\end{subfigure}
\caption{\label{fig:target_comp_effects}Different learning metrics versus the generalization complexity of the target function, when learning with a network of shape $(7,40,40,1)$. Dots represent the means, while the shaded envelope corresponds to piecewise linear interpolation of the standard deviation, over $500$ random initializations and training sets.}
\end{figure}

\begin{figure}[htp]
\centering
\begin{subfigure}[t]{0.49\textwidth}
 \includegraphics[width=\textwidth]{generalization_error_Boolcomp_40_advSGD_new_0_5train_500sample.png}
	\caption{Generalization error of learned functions}
    \label{fig:generror_BC}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
	\includegraphics[width=\textwidth]{BC_comp_learned_vs_BC_comp_0_5train.png}
    \caption{Complexity of learned functions}
    \label{fig:BC_BC}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
	\includegraphics[width=\textwidth]{iters_training_vs_BC_comp_0_5train_b.png}
    \caption{Number of iterations to perfectly fit training set}
    \label{fig:iters_BC}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
	\includegraphics[width=\textwidth]{dists_vs_BC_comp_0_5train.png}
    \caption{Net Euclidean distance traveled in parameter space to fit training set}
    \label{fig:dists_BC}
\end{subfigure}
\caption{\label{fig:target_comp_effects}Different learning metrics versus the Boolean complexity of the target function, when learning with a network of shape $(7,40,40,1)$. Dots represent the means, while the shaded envelope corresponds to piecewise linear interpolation of the standard deviation, over $500$ random initializations and training sets.}
\end{figure}

\begin{figure}[htp]
\centering
\begin{subfigure}[t]{0.49\textwidth}
 \includegraphics[width=\textwidth]{generalization_error_Entropy_40_advSGD_new_0_5train_500sample.png}
	\caption{Generalization error of learned functions}
    \label{fig:generror_Ent}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
	\includegraphics[width=\textwidth]{Ent_learned_vs_Ent_0_5train.png}
    \caption{Complexity of learned functions}
    \label{fig:Ent_Ent}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
	\includegraphics[width=\textwidth]{iters_training_vs_Ent_0_5train_b.png}
    \caption{Number of iterations to perfectly fit training set}
    \label{fig:iters_Ent}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
	\includegraphics[width=\textwidth]{dists_vs_Ent_0_5train.png}
    \caption{Net Euclidean distance traveled in parameter space to fit training set}
    \label{fig:dists_Ent}
\end{subfigure}
\caption{\label{fig:target_comp_effects}Different learning metrics versus the entropy of the target function, when learning with a network of shape $(7,40,40,1)$. Dots represent the means, while the shaded envelope corresponds to piecewise linear interpolation of the standard deviation, over $500$ random initializations and training sets.}
\end{figure}



\subsection{Lempel-Ziv versus Entropy}
\label{Lempel-Ziv-entropy}

To check that the correlation between LZ complexity and generalization is not only because of a correlation with function entropy (which is just a measure of the fraction of inputs mapping to $1$ or $0$, see Section~\ref{complexity_measures}), we observed that for some target functions with maximum entropy (but which are simple when measured using LZ complexity), the network still generalizes better than the unbiased learner, showing that the bias towards simpler functions is better captured by more powerful complexity measures than entropy\footnote{LZ is a better approximation to Kolmogorov complexity than entropy~(\cite{cover2012elements}), but of course LZ can still fail, for example when measuring the complexity of the digits of $\pi$.}. This is confirmed by the results in Fig.~\ref{fig:fixed_ent_generror_comp} where we fix the target function entropy to $1.0$, and observe that the generalization error still exhibits considerable variation, as well as a positive correlation with complexity

\begin{figure}[tph]
\centering
\begin{subfigure}[b]{0.49\textwidth}
 \includegraphics[width=\textwidth]{fixed_ent_generror_LZ.png}
    \caption{}
    \label{fig:fixed_ent_generror_LZ}
\end{subfigure}
~
\begin{subfigure}[b]{0.49\textwidth}
	\includegraphics[width=\textwidth]{fixed_ent_generror_HC.png}
    \caption{}
    \label{fig:fixed_ent_generror_HC}
\end{subfigure}
\caption{\label{fig:fixed_ent_generror_comp}Generalization error of learned function versus the complexity of the target function for target functions with fixed entropy $1.0$, for a network of shape $(7,20,20,1)$. Complexity measures are (a) LZ and (b) generalisation complexity. Here the training set size was of size $64$, but sampled with replacement, and the generalization error is over the whole input space. Note that despite the fixed entropy there is still variation in generalization error, which correlates with the complexity of the function. These figures demonstrate that entropy is a less accurate complexity measure than LZ or generalisation complexity, for predicting generalization performance.}
\end{figure}


\section{Finite-size effects for sampling probability}
\label{finite-size-effects}
Since for a sample of size $N$ the minimum estimated probability is $1/N$, many of the low-probability samples that arise just once may in fact have a much lower probability than suggested. See Figure~\ref{fig:finite_size_effects}), for an illustration of how this finite-size sampling effect manifests with changing sample size $N$.
For this reason, these points are typically removed from plots.
\begin{figure}[htp]
\centering
\includegraphics[width=0.6\textwidth]{finite_size_effects2.png}
\caption{\label{fig:finite_size_effects} Probability (calculated from frequency) versus Lempel-Ziv complexity for a neural network of shape $(7,40,40,1)$, and sample sizes $N=10^6, 10^7, 10^8$. The lowest frequency functions for a given sample size can be seen to suffer from finite-size effects, causing them to have a higher frequency than their true probability.}
\end{figure}

\section{Effect of number of layers on simplicity bias}

In Figure~\ref{fig:prob_comp_layers} we show the effect of the number of layers on the bias (for feedforward neural networks with $40$ neurons per layer). The left figures show the probability of individual functions versus the complexity. The right figure shows the histogram of complexities, weighted by the probability by which the function appeared in the sample of parameters. The histograms therefore show the distribution over complexities when randomly sampling parameters\footnote{using a Gaussian with $1/sqrt{n}$ variance in this case, $n$ being number of inputs to neuron} We can see that between the $0$ layer perceptron and the $2$ layer network there is an increased number of higher complexity functions. This is most likely because of the increasing expressivity of the network. For $2$ layers and above, the expressivity does not significantly change, and instead, we observe a shift of the distribution towards lower complexity.
% Exploring the effect of other architecture choices (like convolutions and skip-connections) is something we aim to do in the future.
% , similar to what was observed in Figure~\ref{fig:CSR_hists} in the main text. 

\begin{figure}[htp]
\centering
\begin{subfigure}[t]{0.33\textwidth}
\includegraphics[width=\textwidth]{prob_LZ_7_1.png}
\caption{\label{fig:prob_LZ_7_1}Perceptron}
\end{subfigure}
~
\begin{subfigure}[t]{0.33\textwidth}
\includegraphics[width=\textwidth]{hist_comp_0_layers.png}
\caption{\label{fig:hist_LZ_7_1} Perceptron}
\end{subfigure}
~
\begin{subfigure}[t]{0.33\textwidth}
\includegraphics[width=\textwidth]{prob_LZ_7_40_1.png}
\caption{\label{fig:prob_comp_layers_40x1}1 hidden layer}
\end{subfigure}
~
\begin{subfigure}[t]{0.33\textwidth}
\includegraphics[width=\textwidth]{hist_comp_1_layers.png}
\caption{\label{fig:hist_comp_layers_40x1}1 hidden layer}
\end{subfigure}
~
\begin{subfigure}[t]{0.33\textwidth}
\includegraphics[width=\textwidth]{prob_LZ_7_40_40_1.png}
\caption{\label{fig:prob_comp_layers_40x2} 2 hidden layers }
\end{subfigure}
~
\begin{subfigure}[t]{0.33\textwidth}
\includegraphics[width=\textwidth]{hist_comp_2_layers.png}
\caption{\label{fig:hist_comp_layers_40x2} 2 hidden layers }
\end{subfigure}
~
\begin{subfigure}[t]{0.33\textwidth}
\includegraphics[width=\textwidth]{cnt_1000000_7_40x5_1_relu_freq_LZ.png}
\caption{\label{fig:prob_comp_layers_40x5} 5 hidden layers }
\end{subfigure}
~
\begin{subfigure}[t]{0.33\textwidth}
\includegraphics[width=\textwidth]{hist_comp_5_layers.png}
\caption{\label{fig:hist_comp_layers_40x5} 5 hidden layers }
\end{subfigure}
~
\begin{subfigure}[t]{0.33\textwidth}
\includegraphics[width=\textwidth]{cnt_1000000_7_40x8_1_relu_freq_LZ.png}
\caption{\label{fig:prob_comp_layers_40x8} 8 hidden layers }
\end{subfigure}
~
\begin{subfigure}[t]{0.33\textwidth}
\includegraphics[width=\textwidth]{hist_comp_8_layers.png}
\caption{\label{fig:hist_comp_layers_40x8} 8 hidden layers }
\end{subfigure}

\caption{\label{fig:prob_comp_layers} Probability versus LZ complexity for networks with different number of layers. Samples are of size $10^6$ (a) \& (b) A perceptron with $7$ input neurons (complexity  is capped at $80$ in (a) to aid comparison with the other figures). (c) \& (d) A network with 1 hidden layer of 40 neurons (e) \& (f) A network with 2 hidden layer of 40 neurons (g) \& (h) A network with 5 hidden layers of 40 neurons each. (i) \& (j)  A network with 8 hidden layers of 40 neurons each }
\end{figure}


% \section{Generalization bounds using SGD}

% In Figure~\ref{fig:gen_bound}, we show the generalization error PAC-Bayes bound (see Section~\ref{pac-bayes} in main text), when training the network using SGD. Note that the range of target function complexities is smaller, because for the most complex functions SGD was not able to perfectly fit the data. The bounds shown here are only for a single training set (rather than averaged over many training sets), and so will show more variance than those in the main text. Furthermore, for each training set we only count runs where SGD was able to perfectly fit the data, which only happened for a small fraction of runs for several target functions. This also causes the bounds to be less good (as the estimate of $P(U)$ is worse).

% \begin{figure}[tph]
% \centering
% \includegraphics[width=0.7\textwidth]{LZ_generror_with_prediction_SGD_0_5train_100000sample_fixed_old_a.png}
% \caption{\label{fig:gen_bound}Generalization error bounds computed for target functions of different frequencies from the estimated probabilities of learned functions (black dots), overlaid over the generalization error for the unbiased learner (red) and neural network (blue), a network of shape $(7,40,40,1)$ trained with SGD. Here we train the network on a single randomly chosen training set, and with $500$ random initializations.  }
% \end{figure}

\section{Bias and the curse of dimensionality}
\label{curse_dimensionality}
We have argued that the main reason deep neural networks are able to generalize is because their implicit prior over functions is heavily biased. We base this claim on PAC-Bayes theory, which tells us that enough bias implies generalization. The contrapositive of this claim is that bad generalization implies small bias. In other words, models which perform poorly on certain tasks relative to deep learning, should show little bias. Here we describe some examples of this, connecting them to the curse of dimensionality. In future work, we plan to explore the converse statement, that small bias implies bad generalization --- one way of approaching this would be via lower bounds matching the PAC-Bayes upper bound.

Complex machine learning tasks require models which are expressive enough to be able to learn the target function. For this reason, before deep learning, the main approach to complex tasks was to use non-parametric models which are infinitely expressible. These include Gaussian processes and other kernel methods. However, unlike deep learning, these models were not successful when applied to tasks where the dimensionality of the input space was very large. We therefore expect that these models show little bias, as they generalize poorly.

Many of these models use kernels which encode some notion of local continuity. For example, the Gaussian kernel ensures that points within a ball of radius $\lambda$ are highly correlated. On the other hand, points separated by a distance greater than $\lambda$ can be very different. Intuitively, we can divide the space into regions of length scale $\lambda$. If the input domain we re considering has $O(1)$ volume, and has dimensionality $d$ (is a subset of $\mathbb{R}^d$), then the volume of each of these regions is of order $\lambda^d$, and the number of these regions is of order $1/\lambda^d$. In the case of binary classification, we can estimate the effective number of functions which the kernel ``prefers'' by constraining the function to take label $0$ or $1$ within each region, but with no further constraint. The number of such functions is $2^{a^d}$, where we let $a:=1/\lambda$. Each of these functions is equally likely, and together they take the bulk of the total probability, so that they have probability close to $2^{-a^d}$, which decreases very quickly with dimension.

Kernels like the Gaussian kernel are biased towards functions which are locally continuous. However, for high dimension $d$, they are not biased \emph{enough}. In particular, as the the probability of the most likely functions grows doubly exponentially with $d$, we expect PAC-Bayes-like bounds to grow exponentially with $d$, quickly becoming vacuous. This argument is essentially a way of understanding the curse of dimensionality from the persective of priors over functions.

\clearpage

\section{Other related work} 
\label{related}

The topic of generalization in neural networks has been extensively studied both in theory and experiment, and the literature is vast.  Theoretical approaches to generalization include classical notions like VC dimension~\cite{baum1989size,bartlett2017nearly} and Rademacher complexity~\cite{sun2016depth}, but also  more modern concepts such as stability \cite{pmlr-v48-hardt16}, robustness~\cite{xu2012robustness}, compression \cite{arora2018stronger} as well as studies on the relation between generalization and properties of stochastic gradient descent (SGD) algorithms~\cite{zhangmusings,soudry2017implicit,advani2017high}.

Empirical studies have also pushed the boundaries proposed by theory,  In particular, in recent work by Zhang et al.~\cite{zhang2016understanding}, it is shown that while deep neural networks are expressive enough to fit randomly labeled data, they can still generalize for data with structure. The generalization error  correlates with the amount of randomization in the labels. A similar result was found much earlier in experiments with smaller neural networks~\cite{franco2006generalization}, where the authors defined a complexity measure for Boolean functions, called generalization complexity (see \SI~\ref{complexity_measures}), which appears to correlate well with the generalization error.

Inspired by the results of Zhang et al.~\cite{zhang2016understanding},  Arpit et al.~\cite{arpit2017closer} propose that the data dependence of generalization for neural networks can be explained because they tend to prioritize learning simple patterns first. The authors show some experimental evidence supporting this hypothesis, and suggest that SGD might be the origin of this implicit regularization. This argument is inspired by the fact that SGD converges to minimum norm solutions for linear models \cite{yao2007early}, but only suggestive empirical results are available for the case of nonlinear models, so that the question remains open \cite{soudry2017implicit}. Wu et al.~\cite{wu2017towards} argue that full-batch gradient descent also generalizes well, suggesting that SGD is not the main cause behind generalization.  It may be that SGD provides some form of implicit regularisation, but here we argue that the exponential bias towards simplicity is so strong that it is likely the main origin of the implicit regularization in the parameter-function map.

The idea of having a bias towards simple patterns has a long history, going back to the philosophical principle of Occam's razor, but having been formalized much more recently in several ways in learning theory. For instance, the concepts of minimum description length (MDL)~\cite{rissanen1978modeling}, Blumer algorithms~\cite{blumer1987occam,wolpert1994relationship}, and universal induction~\cite{ming2014kolmogorov} all rely on a bias towards simple hypotheses. Interestingly, these approaches go hand in hand with non-uniform learnability, which is an area of learning theory which tries to predict data-dependent generalization. For example, MDL tends to be analyzed using structural risk minimization or the related PAC-Bayes approach~\cite{vapnik2013nature,shalev2014understanding}.

Hutter et al.~\cite{lattimore2013no} have shown that the generalization error grows with the target function complexity for a perfect Occam algorithm\footnote{Here what we call a `perfect Occam algorithm' is an algorithm which returns the simplest hypothesis which is consistent with the training data, as measured using some complexity measure, such as Kolmogorov complexity.} which uses Kolmogorov complexity to choose between hypotheses. Schmidhuber applied variants of universal induction to learn neural networks~\cite{schmidhuber1997discovering}.   The simplicity bias from Dingle et al.~\cite{simpbias} arises from a simpler version of the coding theorem of Solomonoff and Levin~\cite{ming2014kolmogorov}.  More theoretical work is needed to make these connections rigorous, but it may be that  neural networks intrinsically approximate universal induction because the parameter-function map results in a prior which approximates the universal distribution.  

%We also build on the theory of non-uniform learnability to understand the effects on generalization.

Other approaches that have been explored for neural networks try to bound generalization by bounding capacity measures like different types of norms of the weights (\cite{neyshabur2015norm,keskar2016large,neyshabur2017exploring,neyshabur2017pac,bartlett2017spectrally,golowich2017size,arora2018stronger}), or unit capacity \cite{neyshabur2018towards}. These capture the behaviour of the real test error (like its improvement with overparametrization (\cite{neyshabur2018towards}), or with training epoch (\cite{arora2018stronger})). However, these approaches have not been able to obtain nonvacuous bounds yet.

Another popular approach to explaining generalisation is based around the idea of flat minima \cite{keskar2016large,wu2017towards}. In~\cite{hochreiter1997flat}, Hochreiter and Schmidhuber argue that flatness could be linked to generalization via the MDL principle. Several experiments also suggest that flatness correlates with generalization. However, it has also been pointed out that flatness is not enough to understand generalization, as sharp minima can also generalize~\cite{dinh2017sharp}. We show in Section~\ref{function_prior} in the main text that simple functions have much larger regions of parameter space producing them, so that they likely give rise to flat minima, even though the same function might also be produced by other sharp regions of parameter space.

Other papers discussing properties of the parameter-function map in neural networks include Montufar et al.~\cite{montufar2014number}, who suggested that looking at the size of parameter space producing functions of certain complexity (measured by the number of linear regions) would be interesting, but left it for future work. In~\cite{poole2016exponential}, Poole et al. briefly look at the sensitivity to small perturbations of the parameter-function map. In spite of these previous works, there is clearly still much scope to study the  properties of the parameter-function map for neural networks.

Other work applying PAC-Bayes theory to deep neural networks include (\cite{dziugaite2017computing,dziugaite2018data,neyshabur2017pac,neyshabur2017exploring}). The work of Dziugaite and Roy is noteworthy in that it also computes non-vacuous bounds. However, their networks differ from the ones used in practice in that they are either stochastic (\cite{dziugaite2017computing}) or trained using a non-standard variant of SGD (\cite{dziugaite2018data}). Admittedly, they only do this because current analysis cannot be rigorously extended to SGD, and further work on that end could make their bounds applicable to realistic networks.

One crucial difference with previous PAC-Bayes work is that we consider the prior \emph{over functions}, rather than the prior over parameters. We think this is one reason why our bounds are tighter than other PAC-Bayes bounds. The many-to-one nature of the parameter-function map in models with redundancy means that: low KL divergence between prior and posterior in parameter space implies low KL divergence between corresponding prior and posterior in function space; conversely, one can have low KL divergence in function space with a large KL divergence in parameter space. Using the PAC-Bayes bound from \cite{pacbayesaveraging}, this implies that bounds using distributions in function space can be tighter. As we explain in Section~\ref{pac-bayes}, we actually use the less-commonly used bound from \cite{mcallester1998some}, which assumes the posterior is the Bayesian posterior, which we argue is a reasonable approximation. This posterior is known to give the tightest PAC-Bayes bounds for a particular prior (\cite{pacbayesaveraging}).


% Our work, however differs significantly from the previous lines of work applying PAC-Bayes, in that we consider the prior \emph{over functions} rather than over parameters. We believe that this new approach can give deeper insight into why deep neural networks generalize.

Finally, our work follows the growing line of work exploring random neural networks \cite{schoenholz2016deep,giryes2016deep,poole2016exponential,schoenholz2017correspondence}, as a way to understand fundamental properties of neural networks, robust to other choices like initialization, objective function, and training algorithm.

% \subsection{Relation to previous work}
% \ard{This section should go into PAC-Bayes section}

% Here we give a brief overview of how our work differs from previous approaches. For more discussion on related work see \SI~\ref{supp-related}. Following the failure of worst-case generalization bounds for deep learning, algorithm and data-dependent bounds have been recently investigated. The main three approaches have been based on algorithmic stability (\cite{pmlr-v48-hardt16}), margin theory (\cite{neyshabur2015norm,keskar2016large,neyshabur2017exploring,neyshabur2017pac,bartlett2017spectrally,golowich2017size,arora2018stronger,neyshabur2018towards}), and PAC-Bayes theory (\cite{dziugaite2017computing,dziugaite2018data,neyshabur2017pac,neyshabur2017exploring}).

% Our approach is based on PAC-Bayes theory. However, one crucial difference with previous PAC-Bayes work is that we consider the prior \emph{over functions}, rather than the prior over parameters. We think this is one reason why our bounds are tighter than other PAC-Bayes bounds. The many-to-one nature of the parameter-function map in models with redundancy means that: low KL divergence between prior and posterior in parameter space implies low KL divergence between corresponding prior and posterior in function space; conversely, one can have low KL divergence in function space with a large KL divergence in parameter space. Using the PAC-Bayes bound from \cite{pacbayesaveraging}, this implies that bounds using distributions in function space can be tighter. As we explain in Section~\ref{pac-bayes}, we actually use the less-commonly used bound from \cite{mcallester1998some}, which assumes the posterior is the Bayesian posterior, which we argue is a reasonable approximation. This posterior is known to give the tightest PAC-Bayes bounds for a particular prior (\cite{pacbayesaveraging}).

% The need to make the bounds algorithm-dependent, has led many to study the properties of the optimization algorithms used to train deep neural networks (\cite{pmlr-v48-hardt16,soudry2017implicit,zhang2018energy,smith2018bayesian,zhangmusings,brutzkus2017sgd,keskar2016large}). However, as we mentioned in the introduction, many neural network optimization algorithms give good performance, and seem to account for differences of only a few percent in the generalization error \cite{wu2017towards,keskar2016large}. To be consistent with this finding, we present an explanation of generalization which makes very mild assumptions about the optimization algorithm. In fact, rather than requiring that it be biased in some special way, we require that it be not too biased in its exploration of parameter space. Instead, the large inductive bias comes from the parameter-function map.

% \pagebreak

% \small {
% \bibliographystyle{iclr2019_conference}
% \bibliography{bib}
% }

% \end{document}

% To put the current work in context, we now review existing approaches to understand generalization of deep learning algorithms. We consider the supervised learning assumptions of i.i.d. samples, and focus on the case of classification. We assume that the output of the algorithm is constrained to lie in some predefined \emph{hypothesis class}, $\hat{f} \in \mathcal{F}$. We also focus on \emph{empirical risk minimization} (ERM) algorithms, which minimize the \emph{training error} on the training sample $S$:

% \begin{equation*}
%     \min\limits_{\hat{f}\in \mathcal{F}} \hat{\epsilon}(\hat{f},S)
% \end{equation*}

% \noindent
% where

% \begin{equation*}
%     \hat{\epsilon}(\hat{f},S) = \frac{1}{m}\sum_{i=1}^m \mathbbm{1}_{\hat{f}(x_i)\neq y_i}
% \end{equation*}

% Most results in learning theory bound generalization error from the training error and some measure of the complexity of the hypothesis class:

% \begin{equation*}
%     \epsilon(\hat{f},f,\mathcal{D}) \lesssim \hat{\epsilon}(\hat{f},S) + \frac{\text{complexity}(\mathcal{F})}{m^\alpha},
% \end{equation*}

% \noindent
% where $m$ is the number of training points, and $1/2 \leq \alpha \leq 1$. It is important to note that the right hand side $\epsilon(\hat{f},f,\mathcal{D})$ depends on $\hat{f}$, $f$, and $\mathcal{D}$, but the bound only depends on these quantities via the training error $\hat{\epsilon}(\hat{f},S)$. The second term in the bound is independent of these quantities (we call such bounds \emph{uniform} on those quantities), and that can make the bound quite loose.

% In the context of (binary) classification, the best bound of this form that can be obtained uses the notion of complexity known as the VC dimension of the class \cite{shalev2014understanding}. For deep neural networks, the VC dimension is proportional to the number of parameters of the network. In the case where the number of parameteres is significantly larger than the number of training points, we thus obtain a bound greater than $1$, which is vacuous, as the generalization error is by definition less than $1$. Because deep learning models are typically overparametrized, it is clear that this type of uniform bound isn't useful for deep learning \cite{zhang2016understanding,neyshabur2017exploring}.

% One extension of the above approach makes the second term in the bound depend on the data distribution $\mathcal{D}$. This results in a data-dependent complexity measure called Rademacher complexity \cite{shalev2014understanding}. Unfortunately, the Rademacher complexity of neural networks is still too large to give useful bounds as evidenced, for instance, by the fact that they can fit data with random labels \cite{zhang2016understanding}. Note that the second term is still independent of $\hat{f}$, which means that it is independent of the particular algorithm we choose.

% It has therefore become clear that to make useful bounds on the generalization error of deep neural networks, we need to make the second term depend on $\hat{f}$ also, so that the bound is allowed to depend on everything that it could depend. There are several proposed approaches to do this. One approach looks at the \emph{margin} of the solution $\hat{f}$, which refers to the closest distance between a point in the training data, and the classification surface (which is the manifold in the input domain separating points classified with different labels). There has been considerable recent work on this front with positive results, as the bounds correlate with the true generalization error \cite{bartlett2017spectrally,neyshabur2017pac,neyshabur2017exploring,neyshabur2018towards}. However, the bounds are still vacuous (much greater than $1$), so that they can't yet explain the observed generalization. Another approach looks at the \emph{stability} of the optimization algorithm to small changes on the training set, and gives a bound that grows with the number of stochastic gradient descent (SGD) iterations performed \cite{hardt2015train}. This bound also fails, given that neural networks actually appear to generalize better with more SGD iterations \cite{hoffer2017train}.

% An approach which shows more promise is based on looking at the ``flatness'' of the minimum of the loss surface (or training error surface) that the training algorithm finds \cite{hochreiter1997flat,keskar2016large}. There have been several arguments showing that minima which are wider generalize better. An extension of this work has managed to obtain some nonvacuous bounds \cite{dziugaite2017computing,dziugaite2018data}. However, the bounds show behavior that differs significantly from the true error.

% In our work we propose to use the PAC-Bayes theorem from \cite{mcallester1998some}. This bound depends on the data and the algorithm. Furthermore the algorithm is assumed to sample functions with a probability proportional to a fixed prior (conditioned on having zero training error, which this theorem assumes is possible). As in Bayesian statistics, this prior captures some ``belief'' about what the true function is, and the bound (roughly) guarantees that if the true function is one which our prior assigns high probability to, the algorithm will generalize well. This prior also allows to capture beliefs about the true function in a more fine-grained way than just assuming it belongs to a given hypothesis class.

% PAC-Bayes can give tighter bounds, the more biased the prior is. We give evidence that suggests that the prior that neural networks implicitly use is extremely biased. This is based on the fact that the parameter-function map is extremely biased. In particular, if you uniformly sample parameters, the distribution over functions is highly nonuniform. Therefore, as long as the algorithm used to sample parameters isn't too biased, the distribution over functions will be biased according to the parameter-function map. As we demonstrate in the paper \cite{perez2018deep}, this gives nonvacuous bounds which follow the same trends as the true generalization error.

